Recursion Aware Modeling and Discovery For Hierarchical Software Event Log Analysis (Extended)

This extended paper presents 1) a novel hierarchy and recursion extension to the process tree model; and 2) the first, recursion aware process model discovery technique that leverages hierarchical information in event logs, typically available for software systems. This technique allows us to analyze the operational processes of software systems under real-life conditions at multiple levels of granularity. The work can be positioned in-between reverse engineering and process mining. An implementation of the proposed approach is available as a ProM plugin. Experimental results based on real-life (software) event logs demonstrate the feasibility and usefulness of the approach and show the huge potential to speed up discovery by exploiting the available hierarchy.

==> gfx/disc/alg-recurse.tex <==
\vspace*{-0.8ex}%
\begin{algorithm}
    \algfontsize
    \caption{Recursion Aware Discovery (\emph{RAD})\label{alg:recurse-discovery}}
    \alginout
        {A hierarchical event log $\symEventLog$}
        {A hierarchical process tree $\symTree$ such that $\symEventLog$ fits
        $\symTree$}
    \algdescript{Extended framework that takes into account
    the named subtree operator~$\treeOpCompOr_f$ and recursion operator~$\treeOpRecurOr_f$.}
    \algname{$RADrun$}{$\symEventLog ,\, \symContextPath$}
\begin{algtab}
    $root = $ \algcall{$RADrun$}{$\symEventLog ,\, \symEmptyTrace$} \\
    \algwhiledo{$\exists \symContextPath : \symEventLog(\symContextPath)$ changed}{
        $model(\symContextPath) = $ \algcall{$RADrun$}{$\symEventLog(\symContextPath),\, \symContextPath$}
    }
    \algforeach{node $P$ in process tree $root$ (including new children)}
        Let $\symContextPath$ be the path of $\treeOpCompOr_f$ names from the root to $P$. \\
        \algifthen{$(\exists f : P = \treeOpCompOr_f) \land \symContextPath \in models$}{
            Set $model(\symContextPath)$ as the child of $P$ 
        }
    \algend
    \algreturn $root$
\end{algtab}
\end{algorithm}
\vspace*{-3.0ex}%
\begin{algorithm}
    \algfontsize
    \caption{Recursion Aware Discovery - single run\label{alg:recurse-discovery-run}}
    \alginout
        {A hierarchical event log $\symEventLog$, and a context path
        $\symContextPath$}
        {A hierarchical process tree $\symTree$ such that $\symEventLog$ fits
        $\symTree$}
    \algdescript{One single run/iteration in the RAD extended framework.}
    \algname{$RADrun$}{$\symEventLog ,\, \symContextPath$}
\begin{algtab}
  \algif{$\forall \symTrace \in \symEventLog : \symTrace = \symEmptyTrace$}
    \emph{// the log is empty or only contains empty traces} \\
    \algreturn $\actSilent$ \\
  \algelseif{$\exists f \in \actAlph : \forall \symTrace \in \symEventLog : 
    \symTrace = \seq{f}$}
    \emph{// the log only has a single low-level activity} \\
    \algreturn $f$ \\
  \algelseif{$\exists f \in \actAlph : \forall \symTrace \in \symEventLog, x \in \symTrace : 
    x[1] = f \land \len{x} > 1$}
    \emph{// all events start with $f$, and there is a lower level in the hierarchy} \\
    \algif{$f \in \symContextPath$}
      \emph{// recursion is detected} \\
      $\symContextPath' = \symContextPath_1 \seqcat \seq{f}$ 
                    \textbf{where} $(\symContextPath_1 \seqcat \seq{f} \seqcat
                    \symContextPath_2) = \symContextPath$ \\
      $\symEventLog(\symContextPath') = \symEventLog(\symContextPath') \cup \seqproject{\symEventLog}{1}$ $\quad$ \emph{// $\seqproject{\symEventLog}{1}$ is added to the sublog for $\symContextPath'$} \\
      \algreturn $\treeOpRecurOr_f$ \\
    \algelse
      \emph{// discovered a named subtree $f$} \\
      $\symEventLog(\symContextPath \seqcat \seq{f}) = \seqproject{\symEventLog}{1}$ $\qquad$ \emph{// $\seqproject{\symEventLog}{1}$ is associated with 
          $\symContextPath' = \symContextPath \seqcat \seq{x}$} \\
      \algreturn $\treeOpCompOr_f$ \\
    \algend
  \algelse
    \emph{// the normal framework cases} \\
    Split $\symEventLog$ into into sublogs $\symEventLog_1, \ldots, \symEventLog_n$, such
    that: \\
    $\exists \treeOp \in \set{\treeOpSeq, \treeOpXor, \treeOpLoop, \treeOpPar}
    : L \subseteq \treeOp^l(\symEventLog_1, \ldots, \symEventLog_n)$ \\
    \algreturn $\treeOp(\funn{RADrun}(\symEventLog_1, \symContextPath), \ldots,
    \funn{RADrun}(\symEventLog_n, \symContextPath))$ \\
  \algend
\end{algtab}
\end{algorithm}
\vspace*{-0.8ex}%


==> gfx/eval-perform/tab-levels.tex <==
\begin{table}[htbp]
  \centering
    \vspace*{-0.1cm}
  \caption{Hierarchy depth for different log preprocessing}
    \vspace*{-0.3cm}
  \begin{tabular}{ l @{\hskip4pt} l
      @{\hskip5pt}
        c @{\hskip5pt}
      l @{\hskip5pt}
      c @{\hskip5pt}
      c @{\hskip1pt}
        c @{\hskip5pt}
      c @{\hskip1pt}
        c @{\hskip5pt}
    }
    & &
    & \multicolumn{3}{p{4.0cm}}{\centering
        Structured Name} 
    & \phantom{a}
    & Nested 
    & \phantom{a}
    \\
    \cmidrule{4-6}
    \cmidrule{8-8}
    & Event Log 
    &
    & Pattern to Split
    & Split
    & Depth 
    &
    & Depth
    &
    \\
   \midrule
   \cite{xeslog:bpic2012} & \textbf{BPIC 2012} & 
      & prefix\_suffix & \_ & 2 & & - & \\
   \cite{xeslog:bpic2013} & \textbf{BPIC 2013} & 
      & activity+lifecycle & + & 2 & & - & \\
   \cite{xeslog:junit412} & \textbf{JUnit 4.12} &
      & package.class.method() & . & 9 & & 25 & \\
  \end{tabular}%
    \vspace*{-0.2cm}
  \label{tab:eval-logs-levels}%
\end{table}%


==> gfx/eval-perform/tab-log-levels.tex <==
\begin{table}[htbp]
\begin{threeparttable}%
  \scriptsize
  \centering
    \vspace*{-0.2cm}
  \caption{Event logs used in the evaluation and their characteristics}
  \begin{tabular}{ 
      @{\hskip4pt} l @{\hskip4pt} l
         @{\hskip3pt} c  @{\hskip3pt}
      D{.}{.}{6.0} @{\hskip2pt}
      D{.}{.}{7.0} @{\hskip2pt}
      D{.}{.}{3.0}  
         @{\hskip3pt} c @{\hskip3pt}
      D{.}{.}{2.0} @{\hskip2pt}
      D{.}{.}{3.0}
         @{\hskip2pt} c @{\hskip4pt}
    }
    & 
    & \phantom{a}
    & \multicolumn{3}{ c }{Log Size}
    & \phantom{a}
    & \multicolumn{2}{ c }{Hierarchy Depth} 
    & \phantom{a} \\
    \cmidrule{4-6}
    \cmidrule{8-9}
    & Event Log 
    &
    & \multicolumn{1}{ c }{\# Traces}
    & \multicolumn{1}{ c }{\# Events}
    & \multicolumn{1}{ c }{\# Acts.}
    &
    & \multicolumn{1}{ c }{Struct.}
    & \multicolumn{1}{ c }{Nested} 
    & \\
   \midrule
   \cite{xeslog:bpic2012} & \textbf{BPIC 2012} &
     & 13,087 & 262,200  & 36 & & 2 & -$\,$ & \\
   \cite{xeslog:bpic2013} & \textbf{BPIC 2013} &
     & 7,554 & 65,533 & 13 & & 2 & -$\,$ & \\
   \cite{xeslog:junit412} & \textbf{JUnit 4.12} &
     & 1 & 946 & 364 & & 9 & 25 & \\
  \end{tabular}%
  \label{tab:eval-logs-performance}%
  \end{threeparttable}%
    \vspace*{-0.2cm}
\end{table}%


==> gfx/eval-perform/tab-logs.tex <==
\begin{table}[htbp]
\begin{threeparttable}%
  \centering
  \caption{Event logs used in performance comparison evaluation}
  \begin{tabular}{ l @{\hskip4pt} l
      D{.}{.}{6.0} 
      D{.}{.}{7.0}  
      D{.}{.}{3.0}  
      D{.}{.}{3.2}
    }
    & Event Log 
    & \multicolumn{1}{ c }{\# Traces}
    & \multicolumn{1}{ c }{\# Events}
    & \multicolumn{1}{ c }{\# Acts}
    & \multicolumn{1}{ c }{Avg. $|$Trace$|$} \\
   \midrule
   \cite{xeslog:bpic2012} & \textbf{BPIC 2012} 
     & 13,087 & 262,200  & 36 & 20.05 \\
   \cite{xeslog:bpic2013} & \textbf{BPIC 2013} 
     & 7,554 & 65,533 & 13 & 8.70 \\
   \cite{xeslog:junit412} & \textbf{JUnit 4.12}
     & 1 & 946 & 364 & 946.00 \\
  \end{tabular}%
  \label{tab:eval-logs-performance}%
  \end{threeparttable}%
    \vspace*{-0.3cm}
\end{table}%


==> gfx/icon_end.tex <==



\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-1.000000, xscale=1.000000, inner sep=0pt, outer sep=0pt]
\begin{scope}[even odd rule,line width=0.800pt]
  \begin{scope}[shift={(-96.0,-480.0)},fill=black]
    \path[fill] (96.0000,480.0000) -- (96.0000,496.0000) -- (112.0000,496.0000) --
      (112.0000,480.0000) -- (96.0000,480.0000) -- cycle(96.0000,480.0000);
  \end{scope}
\end{scope}

\end{tikzpicture}



==> gfx/icon_recurrent.tex <==



\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-1.000000, xscale=1.000000, inner sep=0pt, outer sep=0pt]
  \path (29.8520,2.2970) -- (2.1480,2.2970) -- (2.1480,25.2730) --
    (14.6980,25.2730) -- (13.3910,23.9650) -- (14.9120,22.4450) --
    (4.9760,22.4450) -- (4.9760,5.1240) -- (27.0250,5.1240) -- (27.0250,22.4450)
    -- (20.7640,22.4450) -- (20.7640,18.3010) -- (19.5780,19.4860) --
    (19.5780,19.4510) -- (15.0960,23.9320) -- (15.1140,23.9510) --
    (15.0630,24.0020) -- (20.7640,29.7030) -- (20.7640,25.2730) --
    (29.8520,25.2730) -- cycle;

\end{tikzpicture}



==> gfx/icon_start.tex <==



\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-1.000000, xscale=1.000000, inner sep=0pt, outer sep=0pt]
\path (8.0000,4.0000) -- (8.0000,28.0000) -- (26.0000,16.0000) -- cycle;

\end{tikzpicture}



==> gfx/model/sw-log.tex <==
\begin{table}[htbp]
  \centering
  \caption{A single trace in an example event log corresponding to the program
  in Listing~\ref{lst:running-example}.
  Each column is one event, and each row a different level in the hierarchy. For example,
  $\symHClassifier_0(e_1) = \text{\cf{Main.main()}}$ and $\symHClassifier_2(e_1)
  = \text{\cf{B.stepPre()}}$}
    \begin{tabular}{@{\hskip2pt}r@{\hskip2pt}
    |c@{\hskip4pt}
    |@{\hskip4pt}c@{\hskip4pt}
    |@{\hskip4pt}c@{\hskip4pt}
    |@{\hskip4pt}c@{\hskip4pt}
    |@{\hskip4pt}c@{\hskip4pt}|}
    \multicolumn{1}{c}{}      & \multicolumn{1}{c}{$e_0$} &
    \multicolumn{1}{c}{$e_1$} & \multicolumn{1}{c}{$e_2$} &
    \multicolumn{1}{c}{$e_3$} & \multicolumn{1}{c}{$e_4$} 
    \\ \cline{2-6}
    $\Lambda_0$   &
    \cf{\tiny Main.main()}  & \cf{\tiny Main.main()}  & \cf{\tiny Main.main()} 
    &
    \cf{\tiny Main.main()}    & \cf{\tiny Main.main()}
    \\ \cline{2-6}
    $\Lambda_1$   & \cf{\tiny Main.input()} & \cf{\tiny B.process()}  & \cf{\tiny
    B.process()} &
    \cf{\tiny B.process()}    & \cf{\tiny Main.output()}
    \\ \cline{2-6}
    $\Lambda_2$   &                   & \cf{\tiny B.stepPre()}  & \cf{\tiny B.process()} 
    & \cf{\tiny B.stepPost()}   &
                        \\ \cline{2-6}
    $\Lambda_3$   &                   &                   & \cf{\tiny A.process()}  &     
    &
    \\
                        \cline{2-6}
    \end{tabular}%
  \label{tab:ex-htrace}%
\end{table}%

==> gfx/model/sw-recursion-alg.tex <==
\begin{algorithm}
    \algfontsize
    \caption{Recursion Aware Discovery \label{alg:recursion-discovery}}
    \alginout
        {A hierarchical event log $\symEventLog$}
        {A process tree $\symTree$ such that $\symEventLog$ fits $\symTree$}
    \algdescript{Iteratively discover partial models from (derived logs of)
    $\symEventLog$, using context paths to detect recursion, and yield the combined model.}
    \algname{RecursionAwareDiscovery}{$\symEventLog$}
\begin{algtab}
    $\symContextRecord = \set{\symEmptyTrace \mapsto \msetc{ \tuple{\symTrace,
    \symHClassifier_0} }{\symTrace \in \symEventLog}}$ ; $\symDiscoveryHorizon =
    \set{\symEmptyTrace}$ ; $\symContextModelMap = \emptyset$ \\
    \label{alg:recursion-discovery:runs}\algwhile{$\symDiscoveryHorizon \neq
    \emptyset$} \textbf{Let} $\symContextPath \in \symDiscoveryHorizon$
        ; $\symDiscoveryHorizon = \symDiscoveryHorizon \setminus
        \set{\symContextPath}$ \\
        \label{alg:recursion-discovery:discovery}\textbf{Let} $\symContextModelMap[\symContextPath]$ be the
        model discovered from $\symContextRecord[\symContextPath]$
        \textbf{using:} \\
        \algbegin
            \emph{// (Let $\symEventLog'$ be
            the current (splittled) log, derived from
            $\symContextModelMap[\symContextPath]$) } \\
            \emph{// Named subtree operator $\treeOpCompOr_x$ case:} \\
            \algif{$\exists a \in \actAlph : \forall (\symTrace, \symHClassifier_i) \in \symEventLog', e \in
            \symTrace : \newline
            \symHClassifier_i(e) = a, \symHClassifier_{i+1}(e) \neq
            \symClassUnmapped$}
                \algif{$a \in \symContextPath$}
                    $\symContextPath' = \symContextPath_1 \seqcat \seq{a}$ 
                    \textbf{where} $(\symContextPath_1 \seqcat \seq{a} \seqcat
                    \symContextPath_2) = \symContextPath$ \\
                    \textbf{yield} $\treeOpRecurOr_{a}$ \\
                \algelse
                    $\symContextPath' = \symContextPath \seqcat \seq{a}$ \\
                    \textbf{yield} $\treeOpCompOr_{a}(\treeOpPlaceholder_{\symContextPath'})$ \\
                \algend
                $\symEventLog'' = \msetc{
                \tuple{\symTrace, \symHClassifier_{i+1}} }{ 
                \tuple{\symTrace, \symHClassifier_{i}} \in \symEventLog' } $ \\
                $\symContextRecord[\symContextPath'] =
                (\symContextRecord[\symContextPath'] \setminus \symEventLog'')
                \cup \symEventLog''$ \\
                \label{alg:recursion-discovery:horizon}\algifthen{$\symContextRecord$
                changed}{$\symDiscoveryHorizon = \symDiscoveryHorizon \cup \set{ \symContextPath' }$}
            \algend
            \emph{// Base cases and other splits as per Naive Discovery} \\
        \algend
        %$\symContextModelMap[\symContextPath] = \symTree$ \\
    \algend
    \label{alg:recursion-discovery:return}\algreturn
    $\symContextModelMap[\symEmptyTrace]$ with all $\treeOpPlaceholder_{x}$ substituted by $\symContextModelMap[x]$
    (for all $x \in \setseq{\actAlph}$) \\
\end{algtab}
\end{algorithm}


==> gfx/model/sw-recursion-progress.tex <==
\begin{table}[htbp]
  \centering
  \caption{Example run of Algorithm~\ref{alg:recursion-discovery} for the
  hierarchical event log $\symEventLog = \mset{\seq{x.a, x.x.b}}$. The numbers at the start of the rows denote the iteration run, with
  0 being initialization. The other columns list the values for the key data
  structures at the end of each run. The final model is
  $\treeOpCompOr_{x}(\treeOpXor(b, \treeOpSeq(a, \treeOpRecurOr_{x})))$}
  \vspace*{-0.1cm}
  \begin{tabular}{@{\hskip3pt}r@{\hskip3pt}| P{0.5cm}@{\hskip2pt}L@{\hskip2pt}L@{\hskip2pt}L@{\hskip2pt}L @{\hskip4pt}
    P{1cm}
    @{\hskip4pt} 
    P{0.5cm}@{\hskip2pt}L@{\hskip2pt}L}
    \multicolumn{1}{@{\hskip0pt}c@{\hskip0pt}}{} 
          & \multicolumn{5}{c}{$\symContextRecord$} 
          & \symDiscoveryHorizon 
          & \multicolumn{3}{c}{$\symContextModelMap$}
          \\
    \midrule
    0     & \symEmptyTrace & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_0}
          & ]
          & \set{ \symEmptyTrace }
          & \multicolumn{3}{c}{$\emptyset$}
          \\
    \midrule
    1     & \symEmptyTrace & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_0}
          & ]
          & \set{ \seq{x} }
          & \symEmptyTrace & \mapsto & \treeOpCompOr_{x}(\treeOpPlaceholder_{\seq{x}})
          \\
          & \seq{x} & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_1}
          & ]
          & 
          &         &         &
          \\
    \midrule
    2     & \symEmptyTrace & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_0}
          & ]
          & \set{ \seq{x} }
          & \symEmptyTrace & \mapsto & \treeOpCompOr_{x}(\treeOpPlaceholder_{\seq{x}})
          \\
          & \seq{x} & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_1}
          & ,
          & 
          & \seq{x} & \mapsto & \treeOpSeq(a, \treeOpRecurOr_{x})
          \\
          &         &         &
          & \tuple{\seq{x.x.b}, \symHClassifier_2}
          & ]
          & 
          &         &         &
          \\
    \midrule
    3     & \symEmptyTrace & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_0}
          & ]
          & \emptyset
          & \symEmptyTrace & \mapsto & \treeOpCompOr_{x}(\treeOpPlaceholder_{\seq{x}})
          \\
          & \seq{x} & \mapsto & [
          & \tuple{\seq{x.a, x.x.b}, \symHClassifier_1}
          & ,
          & 
          & \seq{x} & \mapsto & \treeOpXor(b, \treeOpSeq(a, \treeOpRecurOr_{x}))
          \\
          &         &         &
          & \tuple{\seq{x.x.b}, \symHClassifier_2}
          & ]
          & 
          &         &         &
          \\
    \end{tabular}%
  \label{tab:ex-recursion-progress}%
\end{table}%


==> gfx/reduct/reduct-sc.tex <==
\begin{table}[!htb]
  \centering
  \caption{Reduction rules for Statecharts}
    \vspace*{-0.2cm}
   \begin{tabular}{M{30mm} M{30mm}}
    \toprule
        \textbf{Pattern}
      & \textbf{Reduced form}
      \\
    \midrule
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_single-point_pattern.tex}}
         &
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_single-point_reduct.tex}}
      \\
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_point-point_pattern.tex}}
         &
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_point-point_reduct.tex}}
      \\
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_point-simple_pattern.tex}}
         &
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_point-simple_reduct.tex}}
      \\
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_simple-point_pattern.tex}}
         &
         \raisebox{-.9\totalheight}{\input{./gfx/reduct/sc_simple-point_reduct.tex}}
      \\
    \bottomrule
   \end{tabular}
    \vspace*{-0.5cm}
  \label{tab:reduct-sc}%
\end{table}%
